FedD2S: Personalized Data-Free Federated Knowledge Distillation

This paper addresses the challenge of mitigating data heterogeneity among clients within a Federated Learning (FL) framework. The model-drift issue, arising from the noniid nature of client data, often results in suboptimal personalization of a global model compared to locally trained models for each client. To tackle this challenge, we propose a novel approach named FedD2S for Personalized Federated Learning (pFL), leveraging knowledge distillation. FedD2S incorporates a deep-to-shallow layer-dropping mechanism in the data-free knowledge distillation process to enhance local model personalization. Through extensive simulations on diverse image datasets-FEMNIST, CIFAR10, CINIC0, and CIFAR100-we compare FedD2S with state-of-the-art FL baselines. The proposed approach demonstrates superior performance, characterized by accelerated convergence and improved fairness among clients. The introduced layer-dropping technique effectively captures personalized knowledge, resulting in enhanced performance compared to alternative FL models. Moreover, we investigate the impact of key hyperparameters, such as the participation ratio and layer-dropping rate, providing valuable insights into the optimal configuration for FedD2S. The findings demonstrate the efficacy of adaptive layer-dropping in the knowledge distillation process to achieve enhanced personalization and performance across diverse datasets and tasks.

==> jj.tex <==
\relax 
\citation{ISAC}
\citation{FedAvg}
\citation{FedAvg challenges}
\citation{first pFL}
\@writefile{toc}{\contentsline {section}{\numberline {I}\textbf  {Abstract}}{1}{}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {II}\textbf  {Introduction}}{1}{}\protected@file@percent }
\citation{pFedSD}
\citation{feature based improvement}
\citation{DFKD1}
\citation{DFKD4}
\citation{DFKD1}
\citation{FedDTG,FedGEN,FedZKT}
\citation{FedICT}
\citation{FedGEN}
\citation{FedICT}
\citation{Personalization_Layers}
\citation{Personalization_Layers}
\citation{FBDFKD1}
\citation{FBDFKD2}
\citation{FBDFKD3}
\citation{FedAvg}
\citation{FedProx}
\citation{KD}
\citation{KD}
\citation{FedMD}
\citation{FedICT}
\citation{FedGKT}
\@writefile{toc}{\contentsline {section}{\numberline {III}\textbf  {Preliminaries}}{3}{}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {\mbox  {III-A}}\textbf  {Problem Statement}}{3}{}\protected@file@percent }
\newlabel{FL_OP}{{1}{3}}
\newlabel{loss function1}{{2}{3}}
\newlabel{pFL}{{3}{3}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\mbox  {III-B}}\textbf  {Knowledge Distillation}}{3}{}\protected@file@percent }
\newlabel{KD}{{5}{3}}
\citation{FedICT}
\citation{Personalization_Layers}
\citation{FedRep}
\citation{CNN layers}
\citation{Personalization_Layers}
\citation{FedRep}
\@writefile{toc}{\contentsline {section}{\numberline {IV}\textbf  {Methodology: FedD2S Algorithm}}{4}{}\protected@file@percent }
\@writefile{loa}{\contentsline {algorithm}{\numberline {1}{\ignorespaces Proposed FedD2S\relax }}{4}{}\protected@file@percent }
\newlabel{alg}{{1}{4}}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Illustration of the proposed FedD2S workflow.\relax }}{5}{}\protected@file@percent }
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{Fig1}{{1}{5}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\mbox  {IV-A}}\textbf  {Clients-to-Server Distillation}}{5}{}\protected@file@percent }
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\mbox  {IV-A}1}\textbf  {Local Knowledge Extraction}}{5}{}\protected@file@percent }
\citation{Fed Prototype1}
\citation{Fed Prototype2}
\citation{FBDFKD1}
\citation{FBDFKD3}
\citation{FBDFKD1}
\newlabel{dropping layer}{{6}{6}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\mbox  {IV-A}2}\textbf  {Local Knowledge Transferring}}{6}{}\protected@file@percent }
\newlabel{loss function}{{7}{6}}
\newlabel{soft_labe1l}{{8}{6}}
\newlabel{C2S1}{{9}{6}}
\newlabel{C2S2}{{10}{6}}
\newlabel{soft_label2}{{11}{6}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\mbox  {IV-B}}\textbf  {Server-to-Client Distillation}}{6}{}\protected@file@percent }
\citation{FBDFKD1}
\citation{FEMNIST}
\citation{CINIC10}
\citation{CIFAR10}
\citation{CIFAR10}
\citation{FedGEN}
\citation{FedICT}
\citation{FedAvg}
\citation{FedMD}
\citation{Personalization_Layers}
\citation{FedRep}
\citation{FedICT}
\citation{pFedSD}
\@writefile{lot}{\contentsline {table}{\numberline {I}{\ignorespaces A summary of the four distinct soft labels outlined in this paper.\relax }}{7}{}\protected@file@percent }
\newlabel{soft labels}{{I}{7}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\mbox  {IV-B}1} \textbf  {Global Knowledge Extraction}}{7}{}\protected@file@percent }
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\mbox  {IV-B}2}\textbf  {Global Knowledge Transferring}}{7}{}\protected@file@percent }
\newlabel{S2C1}{{12}{7}}
\newlabel{S2C2}{{13}{7}}
\@writefile{toc}{\contentsline {section}{\numberline {V}\textbf  {Simulation Results}}{7}{}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {\mbox  {V-A}}\textbf  {Simulation Setup}}{7}{}\protected@file@percent }
\@writefile{lot}{\contentsline {table}{\numberline {II}{\ignorespaces Average UA (\%) given different data setteing, on various datasets FEMNIST, CINIC10, CIFAR10, and CIFAR100 with participation rate $\rho =0.2$.\relax }}{8}{}\protected@file@percent }
\newlabel{main_acc}{{II}{8}}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces Illustration of data heterogeneity among 10 clients on CIFAR-10 dataset, where the x-axis shows client IDs, the y-axis indicates class IDs, and the size of squares indicates the number of training samples available for each class per client. For comparison, the number of samples for a square is reported in the left figure.\relax }}{8}{}\protected@file@percent }
\newlabel{fig_data_het}{{2}{8}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces Learning curves of average UA (\%) of the proposed FedD2S compared to baseline methods across different datasets, with $\rho =0.2$, $\alpha =0.1$, and $Z_0=3$.\relax }}{9}{}\protected@file@percent }
\newlabel{curves}{{3}{9}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\mbox  {V-B}}\textbf  {Simulation Results and Performance Analysis}}{9}{}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces Comparison of client distribution across accuracy ranges for different datasets—FEMNIST, CIFAR10, CINIC10, and CIFAR100—under the conditions $\alpha =0.1$ and $\rho =0.2$.\relax }}{10}{}\protected@file@percent }
\newlabel{Fairness}{{4}{10}}
\@writefile{lot}{\contentsline {table}{\numberline {III}{\ignorespaces Comparison of Average UA (\%) for the Proposed Method with Head-Model Configurations and MSE Loss Function Across Four Different Layer Dropping Sets.\relax }}{10}{}\protected@file@percent }
\newlabel{headmodel}{{III}{10}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\mbox  {V-C}}\textbf  {Sensitivity Analysis}}{10}{}\protected@file@percent }
\bibcite{ISAC}{1}
\bibcite{FedAvg}{2}
\bibcite{FedAvg challenges}{3}
\bibcite{first pFL}{4}
\bibcite{pFedSD}{5}
\bibcite{feature based improvement}{6}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces The influence of layer dropping dynamics with varying epochs across different datasets.\relax }}{11}{}\protected@file@percent }
\newlabel{epochs}{{5}{11}}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces Average UA (\%) on different distillation intervals $Z_0$ for dataet CIFAR10\relax }}{11}{}\protected@file@percent }
\newlabel{dropping_sets}{{6}{11}}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces Average UA (\%) on FedD2S performance with varying data heterogeneity $\alpha $ for different dropping rate $Z_0$ on CIFAR100\relax }}{11}{}\protected@file@percent }
\newlabel{various distillation intervals}{{7}{11}}
\@writefile{toc}{\contentsline {section}{\numberline {VI}\textbf  {Conclusion}}{11}{}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{References}{11}{}\protected@file@percent }
\bibcite{DFKD1}{7}
\bibcite{DFKD2}{8}
\bibcite{DFKD3}{9}
\bibcite{DFKD4}{10}
\bibcite{FedDTG}{11}
\bibcite{FedGEN}{12}
\bibcite{FedZKT}{13}
\bibcite{FedICT}{14}
\bibcite{Personalization_Layers}{15}
\bibcite{FedRep}{16}
\bibcite{FBDFKD1}{17}
\bibcite{FBDFKD2}{18}
\bibcite{FBDFKD3}{19}
\bibcite{FedProx}{20}
\bibcite{SCAFFOLD}{21}
\bibcite{pFL1}{22}
\bibcite{pFL2}{23}
\bibcite{KD}{24}
\bibcite{Survey_KD}{25}
\bibcite{Responce-Based1}{26}
\bibcite{Responce-Based2}{27}
\bibcite{Relation-Based1}{28}
\bibcite{Relation-Based2}{29}
\bibcite{Model-Compression}{30}
\bibcite{Distributed Model}{31}
\bibcite{Domain-Adaptation}{32}
\bibcite{First_FLKD}{33}
\bibcite{FedMD}{34}
\bibcite{DENSE}{35}
\bibcite{FedGKT}{36}
\bibcite{CNN layers}{37}
\bibcite{Fed Prototype1}{38}
\bibcite{Fed Prototype2}{39}
\bibcite{FEMNIST}{40}
\bibcite{CINIC10}{41}
\bibcite{CIFAR10}{42}
\bibcite{Abstract}{43}
\gdef \@abspage@last{12}

